Wireless Control for Smart Manufacturing: Recent Approaches and Open Challenges

Smart manufacturing aims to overcome the limitations of today's rigid assembly lines by making the material flow and manufacturing process more flexible, versatile, and scalable. The main economic drivers are higher resource and cost efficiency as the manufacturers can more quickly adapt to changing market needs and also increase the lifespan of their production sites. The ability to close feedback loops fast and reliably over long distances among mobile robots, remote sensors, and human operators is a key enabler for smart manufacturing. Thus, this article provides a perspective on control and coordination over wireless networks. Based on an analysis of real-world use cases, we identify the main technical challenges that need to be solved to close the large gap between the current state of the art in industry and the vision of smart manufacturing. We discuss to what extent existing control-over-wireless solutions in the literature address those challenges, including our own approach toward a tight integration of control and wireless communication. In addition to a theoretical analysis of closed-loop stability, practical experiments on a cyber-physical testbed demonstrate that our approach supports relevant smart manufacturing scenarios. The article concludes with a discussion of open challenges and future research directions.

==> img/modeChangeProtocol.tex <==
% !TEX root = ../paper.tex
\begin{figure*}[!tb]
	\centering
	\includegraphics[width=0.8\linewidth]{img/modeChangeProtocol_pdf.pdf}
	%\vspace{-3mm}
	\caption{Operation of mode-change protocol. \capt{The beacon slot is used by the host to inform all nodes about the current mode, the next mode, and when to change to the next mode. The first communication round after a mode change contains no data slots because, in general, all messages generated prior to a mode change are meaningless.}}
	%\vspace{-2mm}
	\label{fig:modeChangeProtocol}
\end{figure*}


==> img/schedulingFramework.tex <==
% !TEX root = ../paper.tex
\begin{figure*}[!tb]
	\centering
	\includegraphics[width=0.75\linewidth]{img/schedulingFramework_pdf.pdf}
	%\vspace{-3mm}
	\caption{Example schedule of application tasks and message transfers between two nodes $P$ and $C$. \capt{Node P senses and acts on a physical system, while node C runs the controller. Time synchronization is provided by \sync line events from communication processors \cp to application processors \ap. Messages are gathered in communication rounds.}}
	% \caption{Example schedule of application tasks and message transfers between two {\dpp}s. \capt{Node P senses and acts on a physical system, while node C runs the controller. The update interval \Tupdate is half the end-to-end delay~\Tdelay.}}
	%\vspace{-2mm}
	\label{fig:schedulingFramework}
\end{figure*}

